Rates of Jets Produced in Association with W and Z Bosons

Presented here is a study of jets produced in association with vector bosons production in pp collisions at \surds = 7 TeV using the full CMS 2010 data set, corresponding to an integrated luminosity of 36 \pm 1.4 pb-1. The transverse energy distribution of the reconstructed leading jets is measured and compared to theoretical expectations. The jet multiplicity distributions are corrected for efficiency and unfolded. The ratios of multiplicities, {\sigma}(V+ \geq n jets)/{\sigma}(V+ \geq (n - 1) jets) and {\sigma}(V+ \geq n jets)/{\sigma}(V) where n stands for number of jets, are also presented along with the first test of the Berends-Giele scaling at \surds = 7 TeV.

==> macros.tex <==
%\renewcommand{\chaptermark}[1]{\markboth{\thechapter\ #1}{}}
\catcode`\@=11 % @ signs are now treated as letters
\DeclareRobustCommand\xdotspace{\futurelet\@let@token\@xdotspace}
\def\@xdotspace{%
  \ifx\@let@token.\else
  \ifx\@let@token\bgroup.\else
  \ifx\@let@token\egroup.\else
  \ifx\@let@token\/.\else
  \ifx\@let@token\ .\else
  \ifx\@let@token~.\else
  \ifx\@let@token!.\else
  \ifx\@let@token,.\else
  \ifx\@let@token:.\else
  \ifx\@let@token;.\else
  \ifx\@let@token?.\else
  \ifx\@let@token/.\else
  \ifx\@let@token'.\else
  \ifx\@let@token).\else
  \ifx\@let@token-.\else
  \ifx\@let@token\@xobeysp.\else
  \ifx\@let@token\space.\else
  \ifx\@let@token\@sptoken.\else
   .\space
   \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi}
\catcode`\@=12 % @ signs are no longer letters
\newcommand{\CL}[1]{$#1\%$~C.L\xdotspace}
\newcommand{\eVdist}{\kern-0.06667em}
\newcommand{\kev}{{\,\text{ke}\eVdist\text{V\/}}}
\newcommand{\mev}{{\,\text{Me}\eVdist\text{V\/}}}
%\newcommand{\gev}{{\,\text{Ge}\eVdist\text{V\/}}}
%\newcommand{\gevc}{{\,\text{Ge}\eVdist\text{V\//\ensuremath{c}}}}
\newcommand{\gevcc}{{\,\text{Ge}\eVdist\text{V\//\ensuremath{c^{2}}}}}
\newcommand{\tev}{{\,\text{Te}\eVdist\text{V\/}}}
%\newcommand{\pbi}{\ensuremath{pb^{-1}}}
\newcommand{\pbi}{\,\text{pb}\ensuremath{^{-1}}}
\newcommand{\fbi}{\,\text{fb}\ensuremath{^{-1}}}
%\newcommand {\ptmiss}{\mbox{\ensuremath{\setminus\hspace{-1.70ex}{P}_t}}}
\newcommand {\ptmiss}{\mbox{$\not\hspace{-0.55ex}{P}_t$}}
\newcommand {\misspt}{\mbox{$\not\hspace{-0.55ex}{P}_t$}}
\newcommand{\Cpp}{C\raisebox{2pt}{\scriptsize{++}}}
\newcommand{\sol}{\ensuremath{S_{0}^{L}}}
\newcommand{\sor}{\ensuremath{S_{0}^{R}}}
\newcommand{\tsor}{\ensuremath{\widetilde{S}_{0}^{R}}}
\newcommand{\sil}{\ensuremath{S_{1}^{L}}}
\newcommand{\viiil}{\ensuremath{V_{1/2}^{L}}}
\newcommand{\viiir}{\ensuremath{V_{1/2}^{R}}}
\newcommand{\tviiil}{\ensuremath{\widetilde{V}_{1/2}^{L}}}
\newcommand{\vol}{\ensuremath{V_{0}^{L}}}
\newcommand{\vor}{\ensuremath{V_{0}^{R}}}
\newcommand{\tvor}{\ensuremath{\widetilde{V}_{0}^{R}}}
\newcommand{\vil}{\ensuremath{V_{1}^{L}}}
\newcommand{\siiil}{\ensuremath{S_{1/2}^{L}}}
\newcommand{\siiir}{\ensuremath{S_{1/2}^{R}}}
\newcommand{\tsiiil}{\ensuremath{\widetilde{S}_{1/2}^{L}}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ud}{\mathrm{d}}
\newcommand{\gimmunnu}{g^{\mu \nu}}
\newcommand{\pimmu}{p^{\mu}}
\newcommand{\pinnu}{p^{\nu}}
\newcommand{\qunnu}{q^{\nu}}
\newcommand{\qummu}{q^{\mu}}
\newcommand{\Tab}[1]{Table~\ref{tab:#1}}
\newcommand{\Tabs}[2]{Tables~\ref{tab:#1} and~\ref{tab:#2}}
\newcommand{\Tabsl}[2]{Tables from ~\ref{tab:#1} to~\ref{tab:#2}}
\newcommand{\Sec}[1]{Sec.~\ref{sec:#1}}
\newcommand{\Secs}[2]{Secs.~\ref{sec:#1} and~\ref{sec:#2}}
\newcommand{\App}[1]{Appendix~\ref{sec:#1}}
\newcommand{\Eq}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\Eqs}[2]{Eqs.~(\ref{eq:#1}) and (\ref{eq:#2})}
\newcommand{\Fig}[2][z]{\mbox{Fig.~\ref{fig:#2}\ifthenelse{\equal{#1}{z}}{}{(#1)}}}
%\newcommand{\Figs}[2][z]{\mbox{Fig.~\ref{fig:#2}\ifthenelse{\equal{#1}{z}}{}{(#1)}}}
\newcommand{\Figs}[2]{Figs.~\ref{fig:#1} and~\ref{fig:#2}}
\newcommand{\Figsl}[2]{Figs. from~\ref{fig:#1} to~\ref{fig:#2}}
\newcommand{\FIG}[2][z]{\mbox{Figure~\ref{fig:#2}\ifthenelse{\equal{#1}{z}}{}{(#1)}}}
\newcommand{\Chap}[1]{Ch.~\ref{ch:#1}}
\newcommand{\spazio}{\rule{0pt}{15pt}}
\newcommand{\spaziosmall}{\rule{0pt}{4pt}}
\newcommand{\mycaption}[1]{\begin{minipage}{0.9\textwidth}\caption{\small{#1}}\end{minipage}}
\newcommand{\mycaptionshort}[2]{\caption[\small{#1}]{\small{#2}}}
\newcommand{\rnge}{\hbox{$\,\text{--}\,$}}
%\newcommand{\cm}{\,\text{cm}}
\newcommand{\DO}{{D{\O}}\xspace}
\newcommand{\cspeed}{\ensuremath{c}}
\newcommand{\alphas}{\ensuremath{\alpha_{S}}}
\newcommand{\lambdaqcd}{\ensuremath{\Lambda_{QCD}}}
\newcommand{\diff}[1]{\ensuremath{\mathrm{d}}#1}
%\newcommand{\pt}{\ensuremath{p_{T}}}
\newcommand{\pthat}{\ensuremath{\hat{p_{T}}}}
%\newcommand{\zjets}{\ensuremath{Z+jets}}
%\newcommand{\kt}{\ensuremath{k_{T}}}
%\newcommand{\kt}{\ensuremath{k_{\perp}}}
\newcommand{\qcut}{\ensuremath{q_{cut}}}
%%%%%particles
\newcommand{\PZ}{\ensuremath{{\mathrm{Z}}}\xspace}
\newcommand{\PV}{\ensuremath{{\mathrm{V}}}\xspace}
\newcommand{\PW}{\ensuremath{{\mathrm{W}}}\xspace}
%\newcommand{\Z}{\ensuremath{Z}\xspace}
\newcommand{\Z}{\PZ}
\newcommand{\photon}{\ensuremath{\gamma}}
%\newcommand{\Wpm}{\ensuremath{W^{\pm{}}}}
\newcommand{\Wp}{\ensuremath{\PW^{+}}\xspace}
\newcommand{\Wm}{\ensuremath{\PW^{-}}\xspace}
\newcommand{\gluon}{\ensuremath{g}}
\newcommand{\zjets}{\ensuremath{\PZ/\gamma^{*}+{\mathrm{jets}}}\xspace}
\newcommand{\zjetsb}{\ensuremath{\PZ+{\mathrm{jets}}}\xspace}
\newcommand{\wjets}{\ensuremath{\PW+{\mathrm{jets}}}\xspace}
\newcommand{\wjetsplus}{\ensuremath{\PW^{+}+{\mathrm{jets}}}\xspace}
\newcommand{\wjetsminus}{\ensuremath{\PW^{-}+{\mathrm{jets}}}\xspace}
\newcommand{\vjets}{\ensuremath{\PV+{\mathrm{jets}}}\xspace}
\newcommand{\vnjets}{\ensuremath{\PV+n~{\mathrm{jets}}}\xspace}
%\newcommand{\W}{\ensuremath{W }\xspace}
\newcommand{\W}{\ensuremath{W }\xspace}
\newcommand{\MN}{\ensuremath{\mu\nu}}%
\newcommand{\ra}{\ensuremath{\rightarrow}}%
\newcommand{\Wmn}{\ensuremath{\PW \ra \MN}}%
\newcommand{\Zmm}{\ensuremath{\PZ \ra \MM}}%
\newcommand{\Wtn}{\ensuremath{\PW \ra \tau\nu}}%
\newcommand{\Ztt}{\ensuremath{\PZ \ra \tau^+\tau^-}}%
\newcommand{\EN}{\ensuremath{\mathrm{e}\nu}}%
\newcommand{\EE}{\ensuremath{\mathrm{e}^+\mathrm{e}^-}}%
\newcommand{\Wen}{\ensuremath{\PW \ra \EN}}%
\newcommand{\Zee}{\ensuremath{\PZ \ra \EE}}%

\newcommand{\ttbar}{\ensuremath{t\bar{t}}}
\newcommand{\MT}{\ensuremath{M_T}}

%%%%%%%%%%%%%%%
%%%%%UNITS
%\newcommand{\mum}{\ensuremath{\rm{\mu}}\text{m}}
%\newcommand{\cm}{\ensuremath{cm}}
\newcommand{\second}{\text{s}}
%\newcommand{\fbi}{\,\text{fb}^{-1}}
%%%%%Generator names
%%\newcommand{\genname}[1]{\texttt{\textbf{#1}}}
\newcommand{\genname}[1]{\textsc{#1}}

\newcommand{\Pythia}{\genname{pythia}\xspace}
\newcommand{\pythia}{\genname{pythia}\xspace}
\newcommand{\PYTHIA}{\genname{pythia}\xspace}
\newcommand{\geant}{\genname{geant}\xspace}
\newcommand{\alpgen}{\genname{AlpGen}\xspace}
\newcommand{\sherpa}{\genname{sherpa}}
\newcommand{\herwig}{\genname{herwig}}
\newcommand{\madgraph}{\genname{MadGraph}\xspace} %/MADEVENT}}
\newcommand{\Madgraph}{\genname{MadGraph}\xspace} %/MADEVENT}}
\newcommand{\MADGRAPH}{\genname{MadGraph}\xspace} %/MADEVENT}}
\newcommand{\mcatnlo}{\genname{MC@NLO}}
\newcommand{\amegic}{\genname{AMEGIC++}}
\newcommand{\apacic}{\genname{APACIC++}}
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\providecommand{\ROOT} {{\textsc{ROOT}}\xspace}
\providecommand{\MINUIT} {{\textsc{MINUIT}}\xspace}

\newcommand{\MYANNOT}[1]{%
%%% commenta questo per segare le MYANNOT
\fbox{\begin{minipage}{3cm}{\tiny{=$\widehat{\rule{2mm}{0pt}}$.$\widehat{\rule{2mm}{0pt}}$= #1}}\end{minipage}}
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\newcommand{\pb}{\ensuremath{\mathrm{pb}}}%
\newcommand{\pp}{\ensuremath{\mathrm{pp}}}%
%\newcommand{\Wo}{\ensuremath{\mathrm{W}}}%
\newcommand{\Wo}{\PW}%
%\newcommand{\Wp}{\ensuremath{\mathrm{W^+}}}%
%\newcommand{\Wm}{\ensuremath{\mathrm{W^-}}}%
%\newcommand{\Zo}{\ensuremath{\mathrm{Z}}}%
\newcommand{\Zo}{\PZ}%
\newcommand{\rts}{\ensuremath{\sqrt{s}}}%
%\newcommand{\ra}{\ensuremath{\rightarrow}}%
%\newcommand{\MN}{\ensuremath{\mu\nu}}%
\newcommand{\MM}{\ensuremath{\mu\mu}}%
\renewcommand{\EE}{\ensuremath{\mathrm{e}^+\mathrm{e}^-}}%
%\newcommand{\EN}{\ensuremath{\mathrm{e}\nu}}%
\newcommand{\LN}{\ensuremath{\ell\nu}}%
\newcommand{\MW}{\ensuremath{\mathrm{m}_\Wo}}%
\newcommand{\MZ}{\ensuremath{\mathrm{m}_\Zo}}%
%\newcommand{\MT}{\ensuremath{\mathrm{M}_T}}%
\newcommand{\MLL}{\ensuremath{M_{\ell^+\ell^-}}}%
\newcommand{\met}{\ensuremath{{E\!\!\!/}_{\mathrm{T}}}\xspace}

%\newcommand{\Wmn}{\ensuremath{\Wo \ra \MN}}%
\newcommand{\Wpmn}{\ensuremath{\Wp \ra \mu^+\nu_\mu}}%
\newcommand{\Wmmn}{\ensuremath{\Wm \ra \mu^-\overline{\nu}_\mu}}%
%\newcommand{\Zmm}{\ensuremath{\Zo \ra \MM}}%
%\newcommand{\Wtn}{\ensuremath{\Wo \ra \tau\nu}}%
%\newcommand{\Ztt}{\ensuremath{\Zo \ra \tau^+\tau^-}}%
\newcommand{\ppZmm}{\pp \ra \Zo(\gamma^*) + X \ra \MM + X}%
\newcommand{\ppWmn}{\pp \ra \Wo + X \ra \MN + X}%
\newcommand{\ppWpmn}{\pp \ra \Wp + X \ra \mu^+\nu_\mu + X}%
\newcommand{\ppWmmn}{\pp \ra \Wm + X \ra \mu^-\overline{\nu}_\mu + X}%

%\newcommand{\Wen}{\ensuremath{\Wo \ra \EN}}%
\newcommand{\Wpen}{\ensuremath{\Wp \ra \mathrm{e}^+\nu_e}}%
\newcommand{\Wmen}{\ensuremath{\Wm \ra \mathrm{e}^-\overline{\nu}_e}}%
%\newcommand{\Zee}{\ensuremath{\Zo \ra \EE}}%
\newcommand{\ppZee}{\pp \ra \Zo(\gamma^*) + X \ra \EE + X}%\
\newcommand{\ppWen}{\pp \ra \Wo + X \ra \EN + X}%
\newcommand{\ppWpen}{\pp \ra \Wp + X \ra \mathrm{e}^+\nu_e  + X}%
\newcommand{\ppWmen}{\pp \ra \Wm + X \ra \mathrm{e}^-\overline{\nu}_e + X}%

\newcommand{\Wln}{\ensuremath{\Wo \ra \LN}}%
\newcommand{\Wpln}{\ensuremath{\Wp \ra \ell^+\nu}}%
\newcommand{\Wmln}{\ensuremath{\Wm \ra \ell^-\overline{\nu}}}%
\newcommand{\Zll}{\ensuremath{\Zo \ra \ell^+ \ell^-}}%
\newcommand{\ppZll}{\pp \ra \Zo(\gamma^*) + X \ra \ell^+ \ell^- + X}%
\newcommand{\ppWln}{\pp \ra \Wo + X \ra \LN + X}%
\newcommand{\ppWpln}{\pp \ra \Wp + X \ra \ell^+\nu  + X}%
\newcommand{\ppWmln}{\pp \ra \Wm + X \ra \ell^-\overline{\nu} + X}%

\newcommand{\Wptn}{\ensuremath{\Wp \ra \tau^+\nu_\tau}}%
\newcommand{\Wmtn}{\ensuremath{\Wm \ra \tau^-\overline{\nu}_\tau}}%

\newcommand{\Wev}{\Wen}
\newcommand{\Wmv}{\Wmn}
\newcommand{\Ztautau}{\Ztt}
\newcommand{\MET}{\met}
\newcommand{\gammaZ}{\ensuremath{\gamma^{*}\Zo}}
\newcommand{\gammaZmm}{\mbox{$ \gamma^{*}/\Zo\rightarrow \MM$}}
\newcommand{\gammaZee}{\mbox{$ \gamma^{*}\Zo\rightarrow e^{+}  e^{-}$}}
\newcommand{\gammaZtt}{\mbox{$ \gamma^{*}\Zo\rightarrow \tau^{+}  \tau^{-}$}}
\newcommand{\gammaZll}{\mbox{$ \gamma^{*}\Zo\rightarrow \ell^{+}  \ell^{-}$}}
\newcommand{\invpb}{\mbox{$\textrm{pb}^{-1}$}}
\newcommand{\invnb}{\mbox{$\textrm{nb}^{-1}$}}
\newcommand{\mz}{\mbox{$ m_{Z}$}}
\newcommand{\hta}{\mbox{$ \eta$}}
\newcommand{\fh}{\mbox{$ \phi$}}
\newcommand{\etot}{\mbox{$ \epsilon_{tot}$}}
\newcommand{\eclustering}{\mbox{$ \epsilon_{clustering}$}}
\newcommand{\etracking}{\mbox{$ \epsilon_{tracking}$}}
\newcommand{\egsfele}{\mbox{$ \epsilon_{gsfele}$}}
\newcommand{\epreselection}{\mbox{$ \epsilon_{preselection}$}}
\newcommand{\eisolation}{\mbox{$ \epsilon_{isolation}$}}
\newcommand{\eclassification}{\mbox{$ \epsilon_{classification}$}}
\newcommand{\eelID}{\mbox{$ \epsilon_{elID}$}}
\newcommand{\etrigger}{\mbox{$ \epsilon_{trigger}$}}

\newcommand{\DE}{$\Delta\eta_{in}$}
\newcommand{\DP}{$\Delta\phi_{in}$}
\newcommand{\SEE}{$\sigma_{\eta\eta}$~}
\newcommand{\SEP}{$\sigma_{\eta\phi}$}
\newcommand{\SPP}{$\sigma_{\phi\phi}$}
\newcommand{\SXY}{$\sigma_{XY}$}
\newcommand{\pth}{\hat{p}_{\perp}}
%\newcommand{\pt}{\ensuremath{p_{T}}~}
\newcommand{\Pt}{\ensuremath{p_{T}}~}
\newcommand{\pt}{\ensuremath{p_{T}}~}
\newcommand{\PT}{\ensuremath{p_{T}}~}
\newcommand{\Et}{\ensuremath{E_{T}}~}
\newcommand{\ET}{\ensuremath{E_{T}}~}
\newcommand{\Lint}{\ensuremath{{\cal L}_{\mathrm{int}}}}

\newcommand{\IRel}{I_{\mathrm{iso}}}
\newcommand{\NBJET}{n_{b-{\mathrm{jet}}}}

\newcommand{\RW}{\ensuremath{R^\pm_\PW}}
\newcommand{\AW}{\ensuremath{A_\PW}}

\newcommand{\ten}[1]{\ensuremath{\times10^#1}}
\newcommand{\GeV}{\textrm{GeV}}

